GenSQL: A Probabilistic Programming System for Querying Generative Models of Database Tables

This article presents GenSQL, a probabilistic programming system for querying probabilistic generative models of database tables. By augmenting SQL with only a few key primitives for querying probabilistic models, GenSQL enables complex Bayesian inference workflows to be concisely implemented. GenSQL's query planner rests on a unified programmatic interface for interacting with probabilistic models of tabular data, which makes it possible to use models written in a variety of probabilistic programming languages that are tailored to specific workflows. Probabilistic models may be automatically learned via probabilistic program synthesis, hand-designed, or a combination of both. GenSQL is formalized using a novel type system and denotational semantics, which together enable us to establish proofs that precisely characterize its soundness guarantees. We evaluate our system on two case real-world studies -- an anomaly detection in clinical trials and conditional synthetic data generation for a virtual wet lab -- and show that GenSQL more accurately captures the complexity of the data as compared to common baselines. We also show that the declarative syntax in GenSQL is more concise and less error-prone as compared to several alternatives. Finally, GenSQL delivers a 1.7-6.8x speedup compared to its closest competitor on a representative benchmark set and runs in comparable time to hand-written code, in part due to its reusable optimizations and code specialization.

==> figures/bdry-semantics.tex <==
%!TEX root=../main.tex
\begin{figure}
%\captionsetup[subfigure]{belowskip=-10pt, aboveskip=0pt}
% \setlength{\abovedisplayskip}{0pt}
% \setlength{\belowdisplayskip}{0pt}
% \setlength{\abovedisplayshortskip}{0pt}
% \setlength{\belowdisplayshortskip}{0pt}
%\setlength{\FrameSep}{0pt}
\begin{framed}
\small
\centering
\textbf{Semantics of Types}
\begin{align*}
\sembdry{\sigma} &= \textstyle \sem{\sigma}\coprod (\{\star_\partial\},
    \mathcal{P}\{\star_\partial\}, \delta_{\{\star_\partial\}}) \\
\tupsem{T[?\id]\tabty{\col_1: \sigma_1,\ldots,\col_n: \sigma_n}}_\partial &=
  \textstyle\left(\prod_{1\leq i\leq n} \sem{\sigma_i}\right)
  \coprod (\{\star_\partial\}, \mathcal{P}\{\star_\partial\},
    \delta_{\{\star_\partial\}}) \\
\tabsem{T[?\id]\tabty{\col_1: \sigma_1,\ldots,\col_n: \sigma_n}}_\partial &=
  \textstyle\bag\left(
    \left(\prod_{1\leq i\leq n} \sem{\sigma_i}\right)
    \coprod (\{\star_\partial\}, \mathcal{P}\{\star_\partial\},
      \delta_{\{\star_\partial\}})\right) \\
\sem{M[?\id]\tabty{\col_1: \sigma_1,\ldots,\col_n: \sigma_n}}_\partial &=
  \textstyle\admissible\left(
    \left(\prod_{1\leq i\leq n} \sem{\sigma_i}\right)
    \coprod (\{\star_\partial\}, \mathcal{P}\{\star_\partial\},
      \delta_{\{\star_\partial\}})
\right)
\end{align*}
\textbf{Semantics of scalar expressions}
$$
\sembdry{c}(\gamma, \delta) = c \qquad
\sembdry{\id.\col_i}(\gamma, \delta) = \pi_i(\delta(\id))
$$
$$
\sembdry{e_1:\sigma_c = e_2:\sigma_c}(\gamma, \delta) = 
\begin{cases}
\star_\bdry & \text{if }\sem{e_1}(\gamma, \delta) = \sem{e_2}(\gamma, \delta) \\
\sem{e_1 = e_2}(\gamma, \delta) & \text{o.w.}
\end{cases}
$$
$$
\sembdry{e_1:\sigma_c < e_2:\sigma_c}(\gamma, \delta) = 
    \sembdry{e_2 > e_1}(\gamma, \delta)
$$
$$
\sembdry{e_1:\sigma_c > e_2:\sigma_c}(\gamma, \delta) = \begin{cases}
    \star_\bdry & \text{if }\sem{e_1}(\gamma,\delta) = \sem{e_2}(\gamma,\delta) \\
    \sem{e_1 > e_2}(\gamma, \delta) & \text{o.w.}
\end{cases}
$$
$$
\sembdry{\op(e_1, \ldots, e_n)}(\gamma, \delta) = \maybe(
\sembdry{e_1}(\gamma,\delta), \ldots, \sembdry{e_n}(\gamma,\delta), 
\op_s(\sembdry{e_1}(\gamma,\delta), \ldots, \sembdry{e_n}(\gamma,\delta)))
$$
\begin{multline*}
\sembdry{\probof c \under m: M\{\col_1:\sigma_1, \ldots, \col_n:\sigma_n\}}(\gamma, \delta) = \\
\begin{cases}
\star_\bdry & \sembdry{m}(\gamma, \delta)\left(\bag_\bdry\left(\prod_{i=1}^n \sem{\sigma}\right)\right) > 0 \\
\maybe(\sembdry{c}(\gamma, \delta), \\
\hspace{4em}\sem{\probof c \under m}(\gamma, \delta)) & \text{o.w.}
\end{cases}
\end{multline*}
\textbf{Semantics of table expressions}
\begin{align*}
\sembdry{\id: T[?\id]\{\cols\}}(\gamma,\delta) &=
  \sem{\id: T[?\id]\{\cols\}}(\gamma,\delta) \\
\sembdry{\rename t \as \id'}(\gamma,\delta) &=
  \sem{\rename t \as \id'}(\gamma,\delta) \\
\sembdry{t_1 \join t_2} (\gamma,\delta) &= \\
  &\hspace{-6em}(\lambda x,y.\maptwo (\lambda r_1,r_2. \maybe(r_1, r_2, (r_1,r_2)))\ x\ y)_*
    (\sembdry{t_1}(\gamma,\delta) \otimes \sembdry{t_2}(\gamma,\delta))\\
\sembdry{t:T[?\id]\{\cols\}\where e}(\gamma,\delta) &=
  \Big(\lambda x.\filter_\bdry (\lambda r. \sembdry{e}(\gamma,\delta[\id\mapsto r]))\ x\Big)_* \sem{t}(\gamma,\delta) \\
\sembdry{\generate m \limit e}(\gamma, \delta) &=
  \llet n=\sembdry{e}(\gamma,\delta)\ \iin\\
    &\hspace{-6em}\Big(\lambda (x_1,\ldots,x_n). \maybe\Big(n, x_1, \ldots, x_n,
      \bigcup_{1\leq i\leq n}\{x_i\}\Big)\Big)_*
      \bigotimes_{1\leq i\leq n}\sembdry{m}(\gamma,\delta)
\end{align*}
\begin{align*}
&\sembdry{\select e_1 \as \col_1,\ldots,e_n \as \col_n \from t:T[?\id]\{\cols\}}
(\gamma,\delta) = \\
&\hspace{2em}\Big(\lambda x. \map \Big(\lambda r. \maybe\Big(\sembdry{e_1}(\gamma,\delta[\id\mapsto r]),
                                             \ldots,
                                             \sembdry{e_n}(\gamma,\delta[\id\mapsto r]), \\
  &\hspace{11.5em} \big(\sem{e_1}(\gamma,\delta[\id\mapsto r]),\ldots,\sem{e_n}(\gamma,\delta[\id\mapsto r])\big)\Big)\Big) \ x \Big)_*
     \sembdry{t}(\gamma, \delta)
\end{align*}
\begin{align*}
&\sembdry{(t:T[?\id]\{\cols\}) \modjoin m}(\gamma,\delta) = \sembdry{t}(\gamma,\delta) \bind
  \Big(\lambda y.\fold (\lambda r,\mu. \mu \bind\\
&\Big(\lambda x. (\lambda \{r'\}. x\cup \{\maybe(r, r', (r,r'))\})_*
\sem{\generate m\limit 1}(\gamma,\delta[\id\mapsto r])\Big) (\return \{\})\ y\Big)
\end{align*}
\end{framed}
\caption{Modified semantics of \iql{} for normalized terms.}
\label{fig:semantics-iql-modified}
\end{figure}
    
\begin{figure}\ContinuedFloat
\small
\centering
\begin{framed}
\textbf{Semantics of Events and Event-0s}
\begin{align*}
\sembdry{\id.\col_i~ \op~ e}(\gamma, \delta) &= \maybe(\sembdry{e}(\gamma, \delta),
\sem{\id.\col_i ~\op~ e}(\gamma, \delta)) \\
\sembdry{c_1 \op\ c_2}(\gamma, \delta) &= \maybe(\sembdry{c_1}(\gamma, \delta),
\sembdry{c_2}(\gamma, \delta), \sem{c_1 \op\ c_2}(\gamma, \delta))
\end{align*}

\textbf{Semantics of \tableModel{} expressions}
$$
\sembdry{\id: M[?\id]\{\cols\}}(\gamma,\delta) = \gamma(\id)
\qquad
\sembdry{\rename m \as \id'}(\gamma,\delta) = \sembdry{m}(\gamma,\delta)
$$
$$
\sembdry{m \given c}(\gamma,\delta) = \begin{cases}
\delta_{\{\star_\bdry\}} & \text{if }\sembdry{c}(\gamma, \delta) = \star_\bdry \\
\sembdry{m}(\gamma, \delta) & \text{otherwise}
\end{cases}
$$

%\begin{align*}
%\end{align*}
\end{framed}
\caption{Modified semantics of \iql{} for normalized terms (continued).}
\label{fig:semantics-iql-modified-2}
\end{figure}


==> figures/gen-code/kepler.tex <==
%!TEX root=../../main.tex
\begin{lstlisting}[language=Julia]
function keplers_law(apogee, perigee)
  GM = 398600.4418; earth_radius = 6378;
  a = (abs(apogee) + abs(perigee)) * 0.5 + earth_radius;
  return 2 * %$\pi$% * sqrt(a^3 / GM) / 60 end;
@gen function custom_model(Perigee_km, Apogee_km)
  out = {:Period} %$\sim$% normal(keplers_law(Perigee_km, Apogee_km), 0.01)
  return out end;
\end{lstlisting}


==> figures/iql-code/anom-example.tex <==
%!TEX root=../../main.tex
\begin{lstlisting}[style=iql]
WITH SELECT STDEV(data.Period_minutes) FROM data AS std_period:
  SELECT data.Period_minutes, data.Class_of_Orbit, 
    data.Perigee_km, data.Apogee_km
  FROM data
  WHERE
      (PROBABILITY OF
        model.Period_minutes > (data.Period_minutes - std_period) AND
        model.Period_minutes < (data.Period_minutes + std_period)
        UNDER model)  
      >
      (PROBABILITY OF
        model.Period_minutes > (data.Period_minutes - std_period) AND
        model.Period_minutes < (data.Period_minutes + std_period)
        UNDER model GIVEN * EXCEPT data.Period_minutes);
\end{lstlisting}


==> figures/iql-code/build.tex <==
%!TEX root=../../main.tex
\begin{lstlisting}[style=iql]
# Synthesize probabilistic
# programs given user-specified
# parameters in parameters.yaml
WITH LOAD 'parameters.yaml'
    AS params:
  BUILD model
  FOR data
  USING params;
\end{lstlisting}


==> figures/iql-code/generate-queries.tex <==
\begin{lstlisting}[style=iql]
SELECT data.Perigee_km, data.Apogee_km 
  FROM data 
GENERATIVE JOIN 
  model.Perigee_km_generated, model.Apogee_km_generated 
  UNDER model;

SELECT Perigee_km, Apogee_km 
  FROM data 
  WHERE data.Period_minutes < 1000
GENERATIVE JOIN 
  model.Perigee_km_generated, model.Apogee_km_generated
  UNDER model 
  GIVEN model.Period_minutes < 1000;
\end{lstlisting}


==> figures/iql-code/parameters.tex <==
%!TEX root=../../main.tex
\begin{lstlisting}[language=yaml, basicstyle=\syntaxcolor\tiny\ttfamily,]
#---- (parameters.yaml) ----#
# Parameters for model building
strategy: Gibbs
number_models_in_ensemble: 100
inference_minutes: 10
\end{lstlisting}


==> figures/iql-code/prediction.tex <==
\begin{lstlisting}[style=iql]
WITH SELECT * FROM data
WHERE rowid <= 1000 AS train_data:
  BUILD default_model FOR train_data AND
  BUILD linear_model  FOR train_data AND

WITH SELECT * FROM data
WHERE rowid > 1000 AS test_data:
  SELECT test_data.period, 
    default_model.period, 
    linear_model.period, 
    custom_model.period
  FROM test_data 
    GENERATIVE JOIN
      default_model.period GIVEN Perigee_km, Apogee_km AND
      linear_model.period  GIVEN Perigee_km, Apogee_km AND
      custom_model.period  GIVEN Perigee_km, Apogee_km
\end{lstlisting}


==> figures/plot-benchmark-optims.tex <==
%!TEX root=../main.tex
\begin{figure}
\captionsetup[subfigure]{skip=0pt,labelfont=footnotesize,textfont=footnotesize}
\begin{subfigure}[t]{0.31\textwidth}
\centering
\includegraphics[width=\textwidth]{figures/plots/optimizations-a.pdf}
\caption{Varying number of conditions and targets in the
\probof queries shown in \cref{tab:runtime}.}
\end{subfigure}
\hfill
\begin{subfigure}[t]{0.31\textwidth}
\centering
\includegraphics[width=\textwidth]{figures/plots/optimizations-b.pdf}
\caption{Varying number of conditions in $\given$ clause for
\generate queries (caching does not apply).}
\label{fig:effect-optim:b}
\end{subfigure}
\hfill
\begin{subfigure}[t]{0.31\textwidth}
\centering
\includegraphics[width=\textwidth]{figures/plots/optimizations-c.pdf}
\caption{Varying number of rows in a data table
used in the $\from$ clause of \select with a $\probof$ query.}
\end{subfigure}

\caption{Runtime comparison between \iql{} (ClojureCat backend) and
raw ClojureCat \citep{CharchutMEngThesis}.}
\label{fig:effect-optim}
\end{figure}


==> figures/plot-case-study-genes-comparison-with-linear-model.tex <==
%!TEX root=../main.tex
\begin{figure}
\captionsetup[subfigure]{skip=0pt}

\begin{subfigure}[t]{\textwidth}
\centering
\includegraphics[width=.55\textwidth]{figures/plots/genes-comp-iql.pdf}
\caption{\footnotesize Comparison of real and generated data from
Bayesian model in \iql{}.}
\label{fig:case-gene-baseline-comparison:iql}
\end{subfigure}

\begin{subfigure}[t]{\textwidth}
\centering
\includegraphics[width=.55\textwidth]{figures/plots/genes-comp-lin-reg.pdf}
\caption{\footnotesize Comparison of real and generated data from
bivariate linear models.}
\label{fig:case-gene-baseline-comparison:linear}
\end{subfigure}

\begin{subfigure}[t]{\textwidth}
\centering
\includegraphics[width=.55\textwidth]{figures/plots/genes-comp-ctgan.pdf}
\caption{\footnotesize Comparison of real and generated data from
a conditional generative adversarial network (CTGAN).}
\label{fig:case-gene-baseline-comparison:gan}
\end{subfigure}

\caption{Comparison to \iql{} models for the gene expression data
with two baseline models: bivariate linear models and conditional
generative adversarial network (CTGAN~\citep{xu2020modeling}).
%  The default configuration of the author's open source
% implementation is used to generate the result in
% \subref{fig:case-gene-baseline-comparison:gan}.
}
\label{fig:case-gene-baseline-comparison}
\end{figure}


==> figures/plot-code-compare-bayesdb.tex <==
%!TEX root=../main.tex
\begin{figure}
\captionsetup[subfigure]{skip=0pt,belowskip=0pt,aboveskip=0pt}
\captionsetup{skip=4pt}
\begin{subfigure}[b]{0.5\textwidth}
\centering
\begin{subfigure}[b]{0.3\textwidth}
\centering
\scriptsize
\begin{tabular}{|ccc|}
\hline
\textbf{a} & \textbf{b} & \textbf{c} \\\hline\hline
$a_0$      & $b_0$      & $c_0$ \\
$a_1$      & $b_1$      & $c_1$ \\
$a_0$      & $b_0$      & $c_0$ \\
$a_0$      & $b_1$      & $c_0$ \\
$\dots$    & $\dots$    & $\dots$\\\hline
\end{tabular}
\caption{Table \texttt{foo}}
\end{subfigure}
\quad
\begin{subfigure}[b]{0.5\textwidth}
\centering
\scriptsize
\begin{tabular}{|ccccc|}
\hline
\textbf{a}&\textbf{b}&\textbf{x}&\textbf{y}&\textbf{z}\\\hline\hline
$a_0$ & $b_1$ & 4.2  & 4.1  & 0.6 \\
$a_1$ & $b_1$ & -4.4 & -5.4 & 0.2\\
$a_1$ & $b_0$ & -3.7 & -6.2 & 0.5\\
$a_1$ & $b_1$ & -6.2 & -4.2 & 0.1\\
\dots&\dots&\dots&\dots&\dots\\\hline
\end{tabular}
\caption{Table \texttt{bar} to build model}
\end{subfigure}

\captionsetup[subfigure]{skip=0pt}
\begin{subfigure}[b]{.8\textwidth}
\centering
\input{figures/iql-code/gen-join}
\caption{\iql{}}
\end{subfigure}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.48\textwidth}
\input{figures/bql-code/gen-join}
\caption{BayesDB}
\end{subfigure}
\caption{Comparison of \iql{} and BayesDB~\citep{mansinghka2015bayesdb} code.
The latter does not support \modjoin.}
\label{fig:compare-code-bayesdb}
\end{figure}


==> figures/plot-code-compare-hand-coded.tex <==
%!TEX root=../main.tex
\begin{figure}
    \centering
    \captionsetup[subfigure]{skip=0pt,belowskip=0pt,aboveskip=0pt}
    \captionsetup{skip=4pt}
    \begin{subfigure}[b]{0.45\textwidth}
     \begin{subfigure}[b]{\textwidth}
         \centering
         \input{figures/iql-code/prob-for-comparison}
         \caption{\iql{}}
         \label{fig:code-proba:a}
     \end{subfigure}
     \begin{subfigure}[b]{\textwidth}
         \centering
        \input{figures/other-code/clojure-prob}
         \caption{ClojureCat (Clojure)}
          \label{fig:code-proba:b}
     \end{subfigure}
    \end{subfigure}\hfill
    \begin{subfigure}[b]{0.5\textwidth}
         \centering
         \input{figures/other-code/sppl-prob}
         \caption{SPPL (Python)}
         \label{fig:code-proba:c}
    \end{subfigure}
    \caption{Comparison of \iql{}, ClojureCat~\citep{CharchutMEngThesis}, and SPPL~\citep{saad2021sppl} code for a conditional probability query.}
    \label{fig:code-proba}
\end{figure}

==> figures/table-program-executions.tex <==
%!TEX root=../main.tex

\begin{figure}[!t]
\centering
\begin{subfigure}[b]{.695\linewidth}
\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{|@{}c@{}|}
\begin{tabular}{lllllll}
\toprule
\textbf{Name}             & \textbf{Country\_of\_Operator} & \textbf{Operator\_Owner} & \textbf{Users}           & \textbf{Purpose}          & \textbf{Class\_of\_Orbit}   & \textbf{Type\_of\_Orbit}      \\ \midrule
Prometheus 1A             & USA                            & Los Alamos Nati          & Military                 & Technology Develo         & LEO                         & Sun-Synchronous               \\
Eutelsat 28A              & Multinational                  & European Teleco          & Commercial               & Communications            & GEO                         & NaN                           \\
SMDC-ONE 1.2              & USA                            & U.S. Army Space          & Military                 & Technology Develo         & LEO                         & NaN                           \\
Lacrosse/Onyx             & USA                            & National Reconn          & Military                 & Surveillance              & LEO                         & Intermediate                  \\
SMOS (Soil Mo             & ESA                            & Centre National          & Government               & Earth Observation         & LEO                         & Sun-Synchronous               \\
Compass G-11              & China (PR)                     & Chinese Defense          & Military                 & Navigation/Global         & GEO                         & NaN                           \\
Echostar 6                & USA                            & Echostar Techno          & Commercial               & Communications            & GEO                         & NaN                           \\
INMARSAT 4 F2             & United Kingdom                 & INMARSAT, Ltd.           & Commercial               & Communications            & GEO                         & NaN                           \\
Eutelsat 25C              & Multinational                  & European Teleco          & Commercial               & Communications            & GEO                         & NaN                           \\
Vinasat 2                 & Vietnam                        & Vietnamese Post          & Government               & Communications            & GEO                         & NaN                           \\[5pt]\midrule
\textbf{Perigee\_km}      & \textbf{Apogee\_km}            & \textbf{Eccentricity}    & \textbf{Period\_minutes} & \textbf{Launch\_Mass\_kg} & \textbf{Dry\_Mass\_kg}      & \textbf{Power\_watts}         \\ \midrule
500                       & 506                            & 0.00044                  & 94.68                    & NaN                       & NaN                         & NaN                           \\
35788                     & 35794                          & 0.00007                  & 1436.10                  & 2950                      & 1375                        & 5900                          \\
483                       & 789                            & 0.02184                  & 97.40                    & 3                         & NaN                         & NaN                           \\
574                       & 676                            & 0.00729                  & 97.21                    & 14500                     & NaN                         & NaN                           \\
759                       & 760                            & 0.00007                  & 100.00                   & 658                       & 630                         & 1065                          \\
35776                     & 35799                          & 0.00027                  & 1436.15                  & 2300                      & NaN                         & NaN                           \\
35775                     & 35798                          & 0.00027                  & 1436.12                  & 3700                      & 1493                        & 11000                         \\
35773                     & 35800                          & 0.00032                  & 1436.11                  & 5458                      & NaN                         & 13000                         \\
35780                     & 35790                          & 0.00012                  & 1436.04                  & 3170                      & 1900                        & 5900                          \\
35742                     & 35776                          & 0.00040                  & 1434.69                  & 2970                      & NaN                         & NaN                           \\[5pt]\midrule
\textbf{Date\_of\_Launch} & \textbf{Anticipated\_Lifetime} & \textbf{Contractor}      & \textbf{Launch\_Site}    & \textbf{Launch\_Vehicle}  & \textbf{longitude\_radians} & \textbf{Inclination\_radians} \\ \midrule
41597                     & NaN                            & Los Alamos Nation        & Wallops Island Fl        & Minotaur 1                & NaN                         & 0.707033                      \\
36958                     & 12                             & Alcatel Space Ind        & Guiana Space Cent        & Ariane 5                  & 0.498466                    & 0.001222                      \\
41165                     & NaN                            & Miltec                   & Vandenberg AFB           & Atlas 5                   & NaN                         & 1.127483                      \\
36755                     & 9                              & Lockheed Martin A        & Vandenberg AFB           & Titan IV                  & NaN                         & 1.186824                      \\
40119                     & 3                              & Thales Alenia Spa        & Plesetsk Cosmodro        & Breeze KM                 & NaN                         & 1.717404                      \\
40963                     & 8                              & Space Technology         & Xichang Satellite        & Long March 3A             & 1.029744                    & 0.032638                      \\
36721                     & 12                             & Lockheed Martin M        & Cape Canaveral           & Atlas 2 AS                & -1.269029                   & 0.001222                      \\
38664                     & 15                             & EADS Astrium             & Sea Launch (Odyss        & Zenit 3SL                 & -0.920836                   & 0.040666                      \\
37580                     & 12                             & Alcatel Space Ind        & Cape Canaveral           & Atlas 2 AS                & 0.445059                    & 0.000349                      \\
41044                     & 15                             & Lockheed Martin C        & Guiana Space Cent        & Ariane 5 ECA              & 2.300344                    & 0.001396                      \\ \bottomrule
\end{tabular}
\end{tabular}
\end{adjustbox}
\captionsetup{skip=5pt}
\caption{Subset of satellites data table showing 21 variables and 10 records}
\end{subfigure}\hfill
\begin{subfigure}[b]{.29\linewidth}
\lstset{morecomment=[l]{\#}}
\begin{lstlisting}[
    frame=single,
    belowskip=0pt,
    framesep=.5pt,
    commentstyle=\color{gray}, basicstyle=\ttfamily\tiny, columns=flexible, keepspaces=True]
# FIRST GROUP OF DEPENDENT VARIABLES
cluster_view_1 ~ categorical(
  {0: 0.945, 1: 0.02, 2: 0.01, ...})
if (cluster_view_1 == 0)
  Eccentricity ~ norm(0.002, 0.01)
elif (cluster_view_1 == 2)
  Eccentricity ~ norm(0.075, 0.015)
elif (cluster_view_1 == 3)
  Eccentricity ~ norm(0.028, 0.017)
...

# SECOND GROUP OF DEPENDENT VARIABLES
cluster_view_2 ~ categorical(
  {0: 0.45, 1: 0.365, 2: 0.01, ...})
if (cluster_view_2 == 0)
  Power_watts     ~ norm(870.32, 877.80)
  Launch_mass_kg  ~ norm(442.08, 528.63)
  Dry_mass_kg     ~ norm(362.45, 321.64)
  Period_miniutes ~ norm(101.67, 56.02)
  Perigee         ~ norm(683.49, 56.02)
  Apogee          ~ norm(742.68, 2411.91)
elif (cluster_view_2 == 1)
  Power_watts     ~ norm(7157.58, 4629.09)
  Launch_mass_kg  ~ norm(3870.96, 1417.09)
  Dry_mass_kg     ~ norm(1921.21, 762.07)
  Period_miniutes ~ norm(1435.63, 57.13)
  Perigee         ~ norm(35820.37, 1434.57)
  Apogee          ~ norm(35701.83, 2548.60)
...
\end{lstlisting}
\captionsetup{skip=5pt}
\caption{Synthesized row generator}
\end{subfigure}

\caption{Synthesizing probabilistic programs that model heterogeneously typed cross-sectional data.}
\label{fig:synthesis}
\end{figure}


==> struct-learning.tex <==
\section{\tableModels{} via Structure Learning}

\iql{}'s \ami{} allows for easy use of well-known structure learning techniques for tabular data. In this section, we present a simple version of this idea to showcase how it is compatible with \iql{}, but more advanced structure learning techniques could be leveraged as well \citep{saad2019bayesian, saad2023sequential,steinruecken2019automatic}. For instance, our experiments leverage a Clojure implementation of CrossCat~\citep{mansinghka2016crosscat}.
In this section, we show a basic concept behind structure learning, and how it can be use to produce \tableModels{} satisfying the \ami{}. 
\begin{itemize}
    \item SPE as CFPG
    \item prior on the grammar
    \item likelihood easy to compute for SPE
    \item MCMC on the SPE space using known things
    \item produces \tableModels{} that satisfy the \ami{}
\end{itemize}

==> tables/anomalies-satellites.tex <==
%!TEX root=../main.tex
\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{llll}
\toprule
 Period\_minutes             & Class\_of\_Orbit & Perigee\_km & Apogee\_km \\\midrule
 \textcolor{red}{\bf   23.9} & GEO              & 35771.0     & 35805.0 \\
 \textcolor{red}{\bf  142.0} & GEO              & 35897.0     & 35909.0 \\
 \textcolor{red}{\bf   14.3} & GEO              & 35770.0     & 35803.0 \\
 \textcolor{red}{\bf   23.9} & GEO              & 35771.0     & 35805.0 \\ \bottomrule
\end{tabular}
\end{adjustbox}

